Benchmarking community detection methods on social media data

Benchmarking the performance of community detection methods on empirical social network data has been identified as critical for improving these methods. In particular, while most current research focuses on detecting communities in data that has been digitally extracted from large social media and telecommunications services, most evaluation of this research is based on small, hand-curated datasets. We argue that these two types of networks differ so significantly that by evaluating algorithms solely on the former, we know little about how well they perform on the latter. To address this problem, we consider the difficulties that arise in constructing benchmarks based on digitally extracted network data, and propose a task-based strategy which we feel addresses these difficulties. To demonstrate that our scheme is effective, we use it to carry out a substantial benchmark based on Facebook data. The benchmark reveals that some of the most popular algorithms fail to detect fine-grained community structure.

==> data/basicModAll.tex <==
\def\infohierdorm{data/infohier-dorm-scores.txt}
\def\infohieryear{data/infohier-year-scores.txt}
\def\infohierUChicagoSmallest{data/infohier-UChicagoSmallest.txt}
\def\louvaintwoadorm{data/louvain02a-dorm-scores.txt}
\def\louvaintwoayear{data/louvain02a-year-scores.txt}
\def\louvaintwoaUChicagoSmallest{data/louvain02a-UChicagoSmallest.txt}
\def\louvaintendorm{data/louvain10-dorm-scores.txt}
\def\louvaintenyear{data/louvain10-year-scores.txt}
\def\louvaintenUChicagoSmallest{data/louvain10-UChicagoSmallest.txt}
\def\linkClusterCombineddorm{data/linkClusterCombined-dorm-scores.txt}
\def\linkClusterCombinedyear{data/linkClusterCombined-year-scores.txt}
\def\linkClusterCombinedUChicagoSmallest{data/linkClusterCombined-UChicagoSmallest.txt}
\def\timescaleCombinedEfivehundreddorm{data/timescaleCombinedE500-dorm-scores.txt}
\def\timescaleCombinedEfivehundredyear{data/timescaleCombinedE500-year-scores.txt}
\def\timescaleCombinedEfivehundredUChicagoSmallest{data/timescaleCombinedE500-UChicagoSmallest.txt}
\def\gceCombinedEfivehundreddorm{data/gceCombinedE500-dorm-scores.txt}
\def\gceCombinedEfivehundredyear{data/gceCombinedE500-year-scores.txt}
\def\gceCombinedEfivehundredUChicagoSmallest{data/gceCombinedE500-UChicagoSmallest.txt}
\def\louvaintenadorm{data/louvain10a-dorm-scores.txt}
\def\louvaintenayear{data/louvain10a-year-scores.txt}
\def\louvaintenaUChicagoSmallest{data/louvain10a-UChicagoSmallest.txt}
\def\linkclusterdorm{data/linkcluster-dorm-scores.txt}
\def\linkclusteryear{data/linkcluster-year-scores.txt}
\def\linkclusterUChicagoSmallest{data/linkcluster-UChicagoSmallest.txt}
\def\gcefifteendorm{data/gce15-dorm-scores.txt}
\def\gcefifteenyear{data/gce15-year-scores.txt}
\def\gcefifteenUChicagoSmallest{data/gce15-UChicagoSmallest.txt}
\def\louvainfiveadorm{data/louvain05a-dorm-scores.txt}
\def\louvainfiveayear{data/louvain05a-year-scores.txt}
\def\louvainfiveaUChicagoSmallest{data/louvain05a-UChicagoSmallest.txt}
\begin{tabular}{lccp{.1cm}ccp{.1cm}lp{2.5cm}p{2.5cm}}
 & \multicolumn{2}{c}{Dorm Accuracies} & & \multicolumn{2}{c}{Year Accuracies} & & \multicolumn{3}{c}{UChicago Stats}\\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-10}
Method & Histogram & Mean & & Histogram & Mean & & \# Comms & Smallest Size Histogram & Mean Smallest Size\\
\midrule
    gce15 & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\gcefifteendorm};
        \end{scope}
    \end{tikzpicture}
    & 46.7 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\gcefifteenyear};
        \end{scope}
    \end{tikzpicture}
    & 64.8 & & 266 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\gcefifteenUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     infohier & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\infohierdorm};
        \end{scope}
    \end{tikzpicture}
    & 32.6 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\infohieryear};
        \end{scope}
    \end{tikzpicture}
    & 58.0 & & 114 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\infohierUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     linkcluster & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\linkclusterdorm};
        \end{scope}
    \end{tikzpicture}
    & 27.2 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\linkclusteryear};
        \end{scope}
    \end{tikzpicture}
    & 37.2 & & 10 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\linkclusterUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain10 & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintendorm};
        \end{scope}
    \end{tikzpicture}
    & 25.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenyear};
        \end{scope}
    \end{tikzpicture}
    & 60.2 & & 27 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain10a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenadorm};
        \end{scope}
    \end{tikzpicture}
    & 27.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenayear};
        \end{scope}
    \end{tikzpicture}
    & 61.2 & & 97 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain05a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveadorm};
        \end{scope}
    \end{tikzpicture}
    & 33.3 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveayear};
        \end{scope}
    \end{tikzpicture}
    & 62.0 & & 151 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain02a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoadorm};
        \end{scope}
    \end{tikzpicture}
    & 42.2 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoayear};
        \end{scope}
    \end{tikzpicture}
    & 63.1 & & 254 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & & \end{tabular}


==> data/modularityAllCombined.tex <==
\def\infohierdorm{data/infohier-dorm-scores.txt}
\def\infohieryear{data/infohier-year-scores.txt}
\def\infohierUChicagoSmallest{data/infohier-UChicagoSmallest.txt}
\def\louvaintwoadorm{data/louvain02a-dorm-scores.txt}
\def\louvaintwoayear{data/louvain02a-year-scores.txt}
\def\louvaintwoaUChicagoSmallest{data/louvain02a-UChicagoSmallest.txt}
\def\louvaintendorm{data/louvain10-dorm-scores.txt}
\def\louvaintenyear{data/louvain10-year-scores.txt}
\def\louvaintenUChicagoSmallest{data/louvain10-UChicagoSmallest.txt}
\def\linkClusterCombineddorm{data/linkClusterCombined-dorm-scores.txt}
\def\linkClusterCombinedyear{data/linkClusterCombined-year-scores.txt}
\def\linkClusterCombinedUChicagoSmallest{data/linkClusterCombined-UChicagoSmallest.txt}
\def\timescaleCombinedEfivehundreddorm{data/timescaleCombinedE500-dorm-scores.txt}
\def\timescaleCombinedEfivehundredyear{data/timescaleCombinedE500-year-scores.txt}
\def\timescaleCombinedEfivehundredUChicagoSmallest{data/timescaleCombinedE500-UChicagoSmallest.txt}
\def\gceCombinedEfivehundreddorm{data/gceCombinedE500-dorm-scores.txt}
\def\gceCombinedEfivehundredyear{data/gceCombinedE500-year-scores.txt}
\def\gceCombinedEfivehundredUChicagoSmallest{data/gceCombinedE500-UChicagoSmallest.txt}
\def\louvaintenadorm{data/louvain10a-dorm-scores.txt}
\def\louvaintenayear{data/louvain10a-year-scores.txt}
\def\louvaintenaUChicagoSmallest{data/louvain10a-UChicagoSmallest.txt}
\def\linkclusterdorm{data/linkcluster-dorm-scores.txt}
\def\linkclusteryear{data/linkcluster-year-scores.txt}
\def\linkclusterUChicagoSmallest{data/linkcluster-UChicagoSmallest.txt}
\def\gcefifteendorm{data/gce15-dorm-scores.txt}
\def\gcefifteenyear{data/gce15-year-scores.txt}
\def\gcefifteenUChicagoSmallest{data/gce15-UChicagoSmallest.txt}
\def\louvainfiveadorm{data/louvain05a-dorm-scores.txt}
\def\louvainfiveayear{data/louvain05a-year-scores.txt}
\def\louvainfiveaUChicagoSmallest{data/louvain05a-UChicagoSmallest.txt}
\begin{tabular}{lccp{.1cm}ccp{.1cm}lp{2.5cm}p{2.5cm}}
 & \multicolumn{2}{c}{Dorm Accuracies} & & \multicolumn{2}{c}{Year Accuracies} & & \multicolumn{3}{c}{UChicago Stats}\\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-10}
Method & Histogram & Mean & & Histogram & Mean & & \# Comms & Smallest Size Histogram & Mean Smallest Size\\
\midrule
    louvain10 & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintendorm};
        \end{scope}
    \end{tikzpicture}
    & 25.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenyear};
        \end{scope}
    \end{tikzpicture}
    & 60.2 & & 27 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain10a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenadorm};
        \end{scope}
    \end{tikzpicture}
    & 27.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenayear};
        \end{scope}
    \end{tikzpicture}
    & 61.2 & & 97 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain05a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveadorm};
        \end{scope}
    \end{tikzpicture}
    & 33.3 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveayear};
        \end{scope}
    \end{tikzpicture}
    & 62.0 & & 151 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvainfiveaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain02a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoadorm};
        \end{scope}
    \end{tikzpicture}
    & 42.2 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoayear};
        \end{scope}
    \end{tikzpicture}
    & 63.1 & & 254 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintwoaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvainAll & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\timescaleCombinedEfivehundreddorm};
        \end{scope}
    \end{tikzpicture}
    & 50.2 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\timescaleCombinedEfivehundredyear};
        \end{scope}
    \end{tikzpicture}
    & 73.6 & & 278 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\timescaleCombinedEfivehundredUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & & \end{tabular}


==> data/modularityMultiscale.tex <==
\def\infohierdorm{data/infohier-dorm-scores.txt}
\def\infohieryear{data/infohier-year-scores.txt}
\def\infohierUChicagoSmallest{data/infohier-UChicagoSmallest.txt}
\def\louvaintwoadorm{data/louvain02a-dorm-scores.txt}
\def\louvaintwoayear{data/louvain02a-year-scores.txt}
\def\louvaintwoaUChicagoSmallest{data/louvain02a-UChicagoSmallest.txt}
\def\louvaintendorm{data/louvain10-dorm-scores.txt}
\def\louvaintenyear{data/louvain10-year-scores.txt}
\def\louvaintenUChicagoSmallest{data/louvain10-UChicagoSmallest.txt}
\def\linkClusterCombineddorm{data/linkClusterCombined-dorm-scores.txt}
\def\linkClusterCombinedyear{data/linkClusterCombined-year-scores.txt}
\def\linkClusterCombinedUChicagoSmallest{data/linkClusterCombined-UChicagoSmallest.txt}
\def\timescaleCombinedEfivehundreddorm{data/timescaleCombinedE500-dorm-scores.txt}
\def\timescaleCombinedEfivehundredyear{data/timescaleCombinedE500-year-scores.txt}
\def\timescaleCombinedEfivehundredUChicagoSmallest{data/timescaleCombinedE500-UChicagoSmallest.txt}
\def\gceCombinedEfivehundreddorm{data/gceCombinedE500-dorm-scores.txt}
\def\gceCombinedEfivehundredyear{data/gceCombinedE500-year-scores.txt}
\def\gceCombinedEfivehundredUChicagoSmallest{data/gceCombinedE500-UChicagoSmallest.txt}
\def\louvaintenadorm{data/louvain10a-dorm-scores.txt}
\def\louvaintenayear{data/louvain10a-year-scores.txt}
\def\louvaintenaUChicagoSmallest{data/louvain10a-UChicagoSmallest.txt}
\def\linkclusterdorm{data/linkcluster-dorm-scores.txt}
\def\linkclusteryear{data/linkcluster-year-scores.txt}
\def\linkclusterUChicagoSmallest{data/linkcluster-UChicagoSmallest.txt}
\def\gcefifteendorm{data/gce15-dorm-scores.txt}
\def\gcefifteenyear{data/gce15-year-scores.txt}
\def\gcefifteenUChicagoSmallest{data/gce15-UChicagoSmallest.txt}
\def\louvainfiveadorm{data/louvain05a-dorm-scores.txt}
\def\louvainfiveayear{data/louvain05a-year-scores.txt}
\def\louvainfiveaUChicagoSmallest{data/louvain05a-UChicagoSmallest.txt}
\begin{tabular}{lccp{.1cm}ccp{.1cm}lp{2.5cm}p{2.5cm}}
 & \multicolumn{2}{c}{Dorm Accuracies} & & \multicolumn{2}{c}{Year Accuracies} & & \multicolumn{3}{c}{UChicago Stats}\\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-10}
Method & Histogram & Mean & & Histogram & Mean & & \# Comms & Smallest Size Histogram & Mean Smallest Size\\
\midrule
    louvain10 & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintendorm};
        \end{scope}
    \end{tikzpicture}
    & 25.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenyear};
        \end{scope}
    \end{tikzpicture}
    & 60.2 & & 27 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & &     louvain10a & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenadorm};
        \end{scope}
    \end{tikzpicture}
    & 27.4 & & 
    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenayear};
        \end{scope}
    \end{tikzpicture}
    & 61.2 & & 97 \\

    \begin{tikzpicture}[xscale=0.01, yscale=0.1]
        \draw[ultra thin, black!50] (1,0)--(100,0);
        \begin{scope}[ycomb, yscale=0.30]
            \draw[black, thin] plot[] file {\louvaintenaUChicagoSmallest};
        \end{scope}
    \end{tikzpicture}
    & 299.0 & & \end{tabular}


==> facebook.tex <==


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:

